DepthSSC: Monocular 3D Semantic Scene Completion via Depth-Spatial Alignment and Voxel Adaptation

The task of 3D semantic scene completion using monocular cameras is gaining significant attention in the field of autonomous driving. This task aims to predict the occupancy status and semantic labels of each voxel in a 3D scene from partial image inputs. Despite numerous existing methods, many face challenges such as inaccurately predicting object shapes and misclassifying object boundaries. To address these issues, we propose DepthSSC, an advanced method for semantic scene completion using only monocular cameras. DepthSSC integrates the Spatial Transformation Graph Fusion (ST-GF) module with Geometric-Aware Voxelization (GAV), enabling dynamic adjustment of voxel resolution to accommodate the geometric complexity of 3D space. This ensures precise alignment between spatial and depth information, effectively mitigating issues such as object boundary distortion and incorrect depth perception found in previous methods. Evaluations on the SemanticKITTI and SSCBench-KITTI-360 dataset demonstrate that DepthSSC not only captures intricate 3D structural details effectively but also achieves state-of-the-art performance.

==> tables/components_abl.tex <==
\iffalse
\begin{table}[t]
        
	\centering
       
	\footnotesize
        %\captionsetup{font=footnotesize}
        
        \resizebox{\columnwidth}{!}{
	\begin{tabular}{l|cc|cc}
		\toprule
		& & &   \multicolumn{2}{c}{SemanticKITTI} \\
		Methods & w/o GAV & w/o ST-GF & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
		Ours & \checkmark  & \checkmark  & \textbf{45.97}  & \textbf{14.59} 	 

		\\
        Depth-GAV   & \scalebox{0.85}[1]{$\times$} & \checkmark & 45.30 \textcolor{blue}{(-0.67)} & 13.74 \textcolor{blue}{(-0.85)}
  	\\

		Depth-ST-GF & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 45.14 \textcolor{blue}{(-0.83)} & 13.55 \textcolor{blue}{(-1.04)}
		\\
		VoxFormer~\cite{li2023voxformer} & \scalebox{0.85}[1]{$\times$} & \scalebox{0.85}[1]{$\times$}  & 44.02 \textcolor{blue}{(-1.95)} & 12.35 \textcolor{blue}{(-2.24)}
		\\
		
		\bottomrule
	\end{tabular}}
 \caption{\textbf{Components ablation.} All of our components boost performance consistently on SemanticKITTI~\cite{behley2019semantickitti}.}
\vspace{-0.6cm}

	\label{tab:ablation_com}

\end{table}
\fi


\begin{table}[t]
	\centering
	\footnotesize
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{l|c|cc|cc}
		\toprule
		& Experiment Type & & &   \multicolumn{2}{c}{SemanticKITTI} \\
		Methods & (Ablation/Alternative) & w/o GAV & w/o ST-GF & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
		Ours & Full Model & \checkmark  & \checkmark  & \textbf{45.97}  & \textbf{14.59} 	 
		\\
          w/o Dynamic Resolution & Ablation & \scalebox{0.85}[1]{$\times$}  & \checkmark  & 45.43 \textcolor{blue}{(-0.54)} & 13.92 \textcolor{blue}{(-0.67)}
        \\
        w/o GAV   & Ablation & \scalebox{0.85}[1]{$\times$} & \checkmark & 45.30 \textcolor{blue}{(-0.67)} & 13.74 \textcolor{blue}{(-0.85)}
  		\\
		w/o ST-GF & Ablation & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 45.14 \textcolor{blue}{(-0.83)} & 13.55 \textcolor{blue}{(-1.04)}
		\\

		\midrule
		\textcolor{red}{Position Offset Prediction (POP)} & Alternative & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 44.85 \textcolor{blue}{(-1.12)} & 13.10 \textcolor{blue}{(-1.49)}
		\\
		\textcolor{red}{Depth-Aware Warping (DAW)} & Alternative & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 44.62 \textcolor{blue}{(-1.35)} & 12.97 \textcolor{blue}{(-1.62)}
		\\
		\textcolor{red}{Deformable Voxel Alignment (DVA)} & Alternative & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 44.50 \textcolor{blue}{(-1.47)} & 12.78 \textcolor{blue}{(-1.81)}
		\\
		VoxFormer~\cite{li2023voxformer} & Baseline & \scalebox{0.85}[1]{$\times$} & \scalebox{0.85}[1]{$\times$}  & 44.02 \textcolor{blue}{(-1.95)} & 12.35 \textcolor{blue}{(-2.24)}
		\\
		\bottomrule
	\end{tabular}}
 \caption{\textbf{Ablation and alternative methods evaluation.} The table compares the performance of ablation studies and alternative methods on SemanticKITTI~\cite{behley2019semantickitti}. ST-GF shows stronger performance than simpler alternatives like POP, DAW, and DVA, highlighting its advantage in capturing spatial dependencies. The addition of the dynamic resolution in GAV also contributes significantly to the final performance.}
\vspace{-0.6cm}
	\label{tab:ablation_com}
\end{table}


\iffalse
\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{minipage}{0.5\textwidth}
        \centering
        \captionsetup{font=footnotesize}
        %\setlength{\tabcolsep}{0.010\linewidth}
        \caption{\textbf{Components ablation.} All of our components boost performance consistently on SemanticKITTI~\cite{behley2019semantickitti}.}
        
        \resizebox{0.9\textwidth}{!}{
	\begin{tabular}{l|cc|cc}
		\toprule
		& & &   \multicolumn{2}{c}{SemanticKITTI} \\
		Methods & w/o GAV & w/o ST-GF & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
		Ours & \checkmark  & \checkmark  & \textbf{45.84}  & \textbf{13.28} 	 

		\\
        Depth-GAV   & \scalebox{0.85}[1]{$\times$} & \checkmark & 45.25 \textcolor{blue}{(-0.59)} & 13.02 \textcolor{blue}{(-0.26)}
  	\\

		Depth-ST-GF & \checkmark  & \scalebox{0.85}[1]{$\times$}   & 44.98 \textcolor{blue}{(-0.86)} & 12.87 \textcolor{blue}{(-0.41)}
		\\
		VoxFormer~\cite{li2023voxformer} & \scalebox{0.85}[1]{$\times$} & \scalebox{0.85}[1]{$\times$}  & 44.02 \textcolor{blue}{(-1.62)} & 12.35 \textcolor{blue}{(-0.93)}
		\\
		
		\bottomrule
	\end{tabular}}

	\label{tab:ablation_com}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        \captionsetup{font=footnotesize}
	\setlength{\tabcolsep}{0.010\linewidth}
	\centering
	\footnotesize
 \caption{\textbf{Ablation study} for STN in ST-GF module.}
 
        \resizebox{0.8\textwidth}{!}{
	\begin{tabular}{l|cc}
		\toprule
		 & \multicolumn{2}{c}{Ours(SemanticKITTI)} \\
		Alignment Method & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
			
	ST-GF   & \textbf{45.84}  & \textbf{13.28} 	
		\\
		
		ICP & 44.23 & 12.57
		\\
		Feature-based Reg.  & 44.37 & 12.68
		\\
		Regularization Matching  &  44.85 & 12.94	
		\\
		
		\bottomrule
	\end{tabular}}
	

	\label{tab:ablation_STN}
    \end{minipage}}
\end{table}

\fi
